Exploring the Camera Bias of Person Re-identification

We empirically investigate the camera bias of person re-identification (ReID) models. Previously, camera-aware methods have been proposed to address this issue, but they are largely confined to training domains of the models. We measure the camera bias of ReID models on unseen domains and reveal that camera bias becomes more pronounced under data distribution shifts. As a debiasing method for unseen domain data, we revisit feature normalization on embedding vectors. While the normalization has been used as a straightforward solution, its underlying causes and broader applicability remain unexplored. We analyze why this simple method is effective at reducing bias and show that it can be applied to detailed bias factors such as low-level image properties and body angle. Furthermore, we validate its generalizability across various models and benchmarks, highlighting its potential as a simple yet effective test-time postprocessing method for ReID. In addition, we explore the inherent risk of camera bias in unsupervised learning of ReID models. The unsupervised models remain highly biased towards camera labels even for seen domain data, indicating substantial room for improvement. Based on observations of the negative impact of camera-biased pseudo labels on training, we suggest simple training strategies to mitigate the bias. By applying these strategies to existing unsupervised learning algorithms, we show that significant performance improvements can be achieved with minor modifications.

==> section/experiment.tex <==
\section{Experiment}
\label{sec:experiment}






\subsection{Experiment setup}

\paragraph{Datasets and evaluation metrics}
The following four person ReID datasets are used: Market-1501~\cite{market}, MSMT17~\cite{msmt}, CUHK03-NP~\cite{cuhk_np}, and PersonX~\cite{personx}, where PersonX is a synthetic dataset.
We follow the new protocol of CUHK03~\cite{cuhk}.
Among them, MSMT17 is known as the most challenging dataset.
VeRi-776~\cite{veri} is additionally used as a vehicle ReID dataset.
Their statistics are provided in Table~\ref{tab:dataset_statistics}. 
For evaluation metrics, the mean average precision (mAP) and cumulative matching characteristics (CMC) Rank-1 (R1), Rank-5 (R5), and Rank-10 (R10) are used.
The NMI scores of the clustering results are also reported as in Section~\ref{sec:motivation}.

\paragraph{Implementation details}
For experiments on the camera-adaptive feature debiasing, we use the pretrained models from their official Github repositories. 
When the model weights are unavailable, we train the models ourselves with the official code.
For experiments on our training strategy for unsupervised learning, we use the DBSCAN~\cite{dbscan} algorithm to obtain pseudo labels.
The person and vehicle images are resized to $384\times128$ and $256\times256$, respectively, following the setup of PPLR.
We train the models on a H100 GPU with batch size 256 and 100 training epochs.



